Get Your Workload in Order: Game Theoretic Prioritization of Database Auditing

For enhancing the privacy protections of databases, where the increasing amount of detailed personal data is stored and processed, multiple mechanisms have been developed, such as audit logging and alert triggers, which notify administrators about suspicious activities; however, the two main limitations in common are: 1) the volume of such alerts is often substantially greater than the capabilities of resource-constrained organizations, and 2) strategic attackers may disguise their actions or carefully choosing which records they touch, making incompetent the statistical detection models. For solving them, we introduce a novel approach to database auditing that explicitly accounts for adversarial behavior by 1) prioritizing the order in which types of alerts are investigated and 2) providing an upper bound on how much resource to allocate for each type. We model the interaction between a database auditor and potential attackers as a Stackelberg game in which the auditor chooses an auditing policy and attackers choose which records to target. A corresponding approach combining linear programming, column generation, and heuristic search is proposed to derive an auditing policy. For testing the policy-searching performance, a publicly available credit card application dataset are adopted, on which it shows that our methods produce high-quality mixed strategies as database audit policies, and our general approach significantly outperforms non-game-theoretic baselines.

==> VIII_conclusion.tex <==
\section{Conclusion}
\label{sec:conc}
Prioritizing the alerts raised by TDMT modules can enable effective auditing of privacy- and security-related incidents.
%This assures the safe operation of the systems processing privacy- and security-related services.
This paper introduced a game theoretic model to represent the strategic interactions between an auditor and a set of potential adversaries.  We showed that discovering the optimal prioritization of alerts is NP-hard,
%In solving the problem, we face two challenges, exponential set of possible orderings of alert types and the combinatorial space of possible choices of thresholds. 
but that several efficient search heuristics can be designed to solve the problem.
%for In face of them, we propose CGGS and ISHM to solve the OAS approximately. The experiments which are set up over a synthetic dataset, show that applying both CGGS and ISHM not only takes much less time and space to run compared with the traditional method, but also leads to a 
Using a controlled, synthetic, dataset, we proved that the heuristics can achieve a performance that is close to the optimal solution.
%tiny gap with the actual optimal solution.
%We investigate the performance of the proposed model on two realistic datasets, Access Logs of VUMC and German Credit Data. 
And, using several different types of datasets illustrated that the heuristics are substantially more effective at prioritization than typical auditng strategies invoked in practice.
%real EMR access log and credic card application and Compared with
%three alternative audit strategies, the proposed model shows obvious advantage in terms of the value of the objective function.
%The proposed model is notable because it is the first general audit model which can be applied in realistic systems for guiding the alert prioritization then capturing adversaries.
We did, however, make several simplifying assumptions regarding the behavior of the adversaries and the parameterization of the variables in the model, but believe that this research provides a foundation for further investigation in alert priortization games. 
